Error-margin Analysis for Hidden Neuron Activation Labels

Understanding how high-level concepts are represented within artificial neural networks is a fundamental challenge in the field of artificial intelligence. While existing literature in explainable AI emphasizes the importance of labeling neurons with concepts to understand their functioning, they mostly focus on identifying what stimulus activates a neuron in most cases, this corresponds to the notion of recall in information retrieval. We argue that this is only the first-part of a two-part job, it is imperative to also investigate neuron responses to other stimuli, i.e., their precision. We call this the neuron labels error margin.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}


% ------- Discussion Points ----- 
% 1. 


==> sections/preliminaries.tex <==
\section{Preliminaries}



==> sections/results.tex <==
\section{Results}
\label{sec:results}

% 1. Performance metrics are used to evaluate the results and how these metrics quantify the effectiveness or quality of the proposed approach?
%Our study aimed to evaluate the reliability and generalizability of \textit{error-margins} (Non-TLA\%) obtained from the Google Images dataset, comparing them with the ADE20k dataset. Through a meticulous statistical evaluation, we gained valuable insights into the performance of our methodology.

Our findings suggest that our methodology for assigning \textit{error-margins} for image predictions is not only reliable but also generalizable across diverse datasets, confirmed by statistical evaluation. 

Table~\ref{tab:stats_eval} demonstrates a consistent trend of decreased Non-TLA\% in the ADE20k dataset compared to Google Images across various threshold categories. Among the 33 hypotheses tested for the category of non-target activations $>$ 0, 13 were rejected at a significance level of p $<$ 0.05. Similarly, for the category of non-target activations $>$ 20\%, 15 hypotheses were rejected at the same significance level. In the case of non-target activations $>$ 40\%, 21 hypotheses were rejected, while for non-target activations $>$ 60\%, 23 hypotheses were rejected, all at a p-value $<$ 0.05. These findings underscore a consistent and statistically significant decrease in non-target activations in the ADE20k dataset, indicating its potential for robust image analysis tasks.

The Wilcoxon signed rank test results further reinforce this trend. Across various thresholds, the test consistently indicated a decrease in non-target activations in the ADE20k dataset compared to Google Images. This trend was particularly evident when considering all threshold categories together, where the p-value was found to be $<$ 0.05, leading to the rejection of the null hypothesis. This suggests that the error estimates obtained from the Google image data are reliable and are either maintained or even surpassed by the ADE20k images, highlighting the potential of leveraging ADE20k for image analysis tasks, particularly in scenarios where minimizing error rates is crucial. This comparative analysis offers valuable insights for refining image analysis methodologies and informs future research directions in this domain.


% 3a. Main findings or results obtained from the experiments [AD]


% 4. key successes or achievements of the approach


% 5. How do these results compare to expectations or prior hypotheses

